Millimeter-Scale Absolute Carrier Phase-Based Localization in Multi-Band Systems

Localization is a key feature of future Sixth Generation (6G) net-works with foreseen accuracy requirements down to the millimeter level, to enable novel applications in the fields of telesurgery, high-precision manufacturing, and others. Currently, such accuracy requirements are only achievable with specialized or highly resource-demanding systems, rendering them impractical for more wide-spread deployment. In this paper, we present the first system that enables low-complexity and low-bandwidth absolute 3D localization with millimeter-level accuracy in generic wireless networks. It performs a carrier phase-based wireless localization refinement of an initial location estimate based on successive location-likelihood optimization across multiple bands. Unlike previous phase unwrapping methods, our solution is one-shot. We evaluate its performance collecting ~350, 000 measurements, showing an improvement of more than one order of magnitude over classical localization techniques. Finally, we will open-source the low-cost, modular FR3 front-end that we developed for the experimental campaign.

==> figures/sysmodel.tex <==
\colorlet{sub6color}{orange}
\colorlet{fr3color}{blue}
\colorlet{mmcolor}{black}
\colorlet{classcolor}{green}




\def\boxwidth{0.95*\linewidth}
\def\boxheight{0.7*\linewidth}
\def\coherentscalex{1.2*0.4*\boxwidth}
\def\coherentscaley{1.2*0.6*\boxheight}



\begin{tikzpicture}[spy using outlines={circle, magnification=4, size=1.3cm, connect spies}]

\coordinate (enhanceBL) at (0.4 *\boxwidth, 0.1 * \boxheight);
\coordinate (enhanceTR) at (0.95 *\boxwidth, 0.75 * \boxheight);
\coordinate  (enhanceTL) at at (enhanceTR-|enhanceBL);
\coordinate  (enhanceBR) at at (enhanceBL-|enhanceTR);

\coordinate (classBL) at  (0.4 *\boxwidth, 0.8 * \boxheight);
\coordinate (classTR) at  (0.95 *\boxwidth, 0.9 * \boxheight);
\coordinate  (classTL) at at (classTR-|classBL);
\coordinate  (classBR) at at (classBL-|classTR);

\coordinate (FR1BL) at  (0.05 *\boxwidth, 0.7 * \boxheight);
\coordinate (FR1TR) at(0.3 *\boxwidth, 0.9 * \boxheight);
\coordinate  (FR1TL) at at (FR1TR-|FR1BL);
\coordinate  (FR1BR) at at (FR1BL-|FR1TR);

\coordinate (FR3BL) at  (0.05 *\boxwidth, 0.4 * \boxheight);
\coordinate (FR3TR) at  (0.3 *\boxwidth, 0.6 * \boxheight);
\coordinate  (FR3TL) at at (FR3TR-|FR3BL);
\coordinate  (FR3BR) at at (FR3BL-|FR3TR);

\coordinate (FR2BL) at  (0.05 *\boxwidth, 0.1 * \boxheight);
\coordinate (FR2TR) at  (0.3 *\boxwidth, 0.3 * \boxheight); 
\coordinate  (FR2TL) at at (FR2TR-|FR2BL);
\coordinate  (FR2BR) at at (FR2BL-|FR2TR);



\filldraw [fill=cyan!20!white, draw=black, rounded corners] (0,0) rectangle (\boxwidth,\boxheight);
\filldraw [fill=yellow!10!white, draw=black, rounded corners] (enhanceBL) rectangle  (enhanceTR);
\node[below, anchor= north east] at ($(enhanceTL)!.99!(enhanceTR)$) {Coherent enahncment};
\filldraw [fill=classcolor!20!white, draw=black, rounded corners] (classBL) rectangle (classTR)  node[pos=.5] {Classical localization};


\filldraw [fill=sub6color!20!white, draw=black, rounded corners] (FR1BL)  rectangle  (FR1TR) node[pos=.5] {Band 1};
\filldraw [fill=fr3color!20!white, draw=black, rounded corners] (FR3BL) rectangle (FR3TR)  node[pos=.5] {Band 2};
\filldraw [fill=mmcolor!20!white, draw=black, dashed, rounded corners] (FR2BL)  rectangle  (FR2TR) node[pos=.5] {Band 3};






%baseband links
\draw[-stealth, green!50!black] ($(FR1TR)!.3!(FR1BR)$) node[left] {\tiny BB} --  ($(classTL)!.25!(classBL)$);
\draw[-stealth, green!50!black] ($(FR3TR)!.3!(FR3BR)$) node[left] {\tiny BB}--  ($(classTL)!.5!(classBL)$);
\draw[-stealth, green!50!black, dashed] ($(FR2TR)!.3!(FR2BR)$) node[left] {\tiny BB} --  ($(classTL)!.75!(classBL)$);


\coordinate (step1) at (0.15*\coherentscalex,-0.3*\coherentscaley);

\draw[-stealth] ($(enhanceTL)+(step1)$) -- ++ (0, 0.2 * \coherentscalex) node[left] {\tiny Y};
\draw[-stealth] ($(enhanceTL)+(step1)$) -- ++ (0.2 * \coherentscalex, 0) node[below] {\tiny X};



\filldraw[classcolor!20!white] ($(enhanceTL)+(step1)+(0.1*\coherentscalex, 0.11*\coherentscalex)$) circle (0.04 * \coherentscalex) ;

\filldraw[sub6color!30!white] ($(enhanceTL)+(step1)+(0.05*\coherentscalex, 0.05*\coherentscalex)$) circle (0.02 * \coherentscalex) ;
\filldraw[sub6color!30!white] ($(enhanceTL)+(step1)+(0.1*\coherentscalex, 0.1*\coherentscalex)$) circle (0.02 * \coherentscalex) ;
\filldraw[sub6color!30!white] ($(enhanceTL)+(step1)+(0.15*\coherentscalex, 0.15*\coherentscalex)$) circle (0.02 * \coherentscalex) ;
\filldraw[sub6color!30!white] ($(enhanceTL)+(step1)+(0.15*\coherentscalex, 0.05*\coherentscalex)$) circle (0.02 * \coherentscalex) ;
\filldraw[sub6color!30!white] ($(enhanceTL)+(step1)+(0.05*\coherentscalex, 0.15*\coherentscalex)$) circle (0.02 * \coherentscalex) ;


\draw ($(enhanceTL)+(step1)+(0.05*\coherentscalex, 0.05*\coherentscalex)$) node[cross=0.015 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step1)+(0.15*\coherentscalex, 0.15*\coherentscalex)$) node[cross=0.015 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step1)+(0.15*\coherentscalex, 0.05*\coherentscalex)$) node[cross=0.015 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step1)+(0.05*\coherentscalex, 0.15*\coherentscalex)$) node[cross=0.015 * \coherentscalex, red]{};


\node[green] at ($(enhanceTL)+(step1)+(0.1*\coherentscalex, 0.1*\coherentscalex)$) {\tiny $\checkmark$};

\coordinate (topclasscircle) at ($(enhanceTL)+(step1)+(0.1*\coherentscalex, 0.11*\coherentscalex) + (0,0.04 * \coherentscalex) $);

\draw[-stealth, black] (classBR-|topclasscircle) -- (topclasscircle); 
\node[right] at ($ (classBR-|topclasscircle)!.15!(topclasscircle)$)  {\tiny Initial location};


\coordinate (step2) at (0.35*\coherentscalex,-0.55*\coherentscaley);

\draw[-stealth] ($(enhanceTL)+(step2)$) -- ++ (0, 0.2 * \coherentscalex) node[left] {\tiny Y};
\draw[-stealth] ($(enhanceTL)+(step2)$) -- ++ (0.2 * \coherentscalex, 0) node[below] {\tiny X};

\filldraw[classcolor!20!white] ($(enhanceTL)+(step2)+(0.1*\coherentscalex, 0.11*\coherentscalex)$) circle (0.04 * \coherentscalex) ;
\filldraw[sub6color!30!white] ($(enhanceTL)+(step2)+(0.1*\coherentscalex, 0.1*\coherentscalex)$) circle (0.02 * \coherentscalex) ;


\draw[line width = 2, ->] ($(enhanceTL)+(step1) + (0.05 * \coherentscalex, -0.05 * \coherentscalex)$) |- ($(enhanceTL)+(step2) + (-0.05 * \coherentscalex, 0.1 * \coherentscalex)$);

\filldraw[fr3color!30!white] ($(enhanceTL)+(step2)+(0.06*\coherentscalex, 0.06*\coherentscalex)$) circle (0.012 * \coherentscalex) ;
\filldraw[fr3color!30!white] ($(enhanceTL)+(step2)+(0.06*\coherentscalex, 0.095*\coherentscalex)$) circle (0.012 * \coherentscalex) ;
\filldraw[fr3color!30!white] ($(enhanceTL)+(step2)+(0.095*\coherentscalex, 0.06*\coherentscalex)$) circle (0.012 * \coherentscalex) ;
\filldraw[fr3color!30!white] ($(enhanceTL)+(step2)+(0.095*\coherentscalex, 0.095*\coherentscalex)$) circle (0.012 * \coherentscalex) ;
\filldraw[fr3color!30!white] ($(enhanceTL)+(step2)+(0.130*\coherentscalex, 0.095*\coherentscalex)$) circle (0.012 * \coherentscalex) ;
\filldraw[fr3color!30!white] ($(enhanceTL)+(step2)+(0.130*\coherentscalex, 0.130*\coherentscalex)$) circle (0.012 * \coherentscalex) ;
\filldraw[fr3color!30!white] ($(enhanceTL)+(step2)+(0.095*\coherentscalex, 0.130*\coherentscalex)$) circle (0.012 * \coherentscalex) ;
\filldraw[fr3color!30!white] ($(enhanceTL)+(step2)+(0.06*\coherentscalex, 0.130*\coherentscalex)$) circle (0.012 * \coherentscalex) ;
\filldraw[fr3color!30!white] ($(enhanceTL)+(step2)+(0.130*\coherentscalex, 0.06*\coherentscalex)$) circle (0.012 * \coherentscalex) ;




\draw ($(enhanceTL)+(step2)+(0.06*\coherentscalex, 0.06*\coherentscalex)$) node[cross=0.01 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step2)+(0.06*\coherentscalex, 0.095*\coherentscalex)$) node[cross=0.01 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step2)+(0.095*\coherentscalex, 0.06*\coherentscalex)$) node[cross=0.01 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step2)+(0.130*\coherentscalex, 0.095*\coherentscalex)$) node[cross=0.01 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step2)+(0.130*\coherentscalex, 0.130*\coherentscalex)$) node[cross=0.01 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step2)+(0.095*\coherentscalex, 0.130*\coherentscalex)$) node[cross=0.01 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step2)+(0.06*\coherentscalex, 0.130*\coherentscalex)$) node[cross=0.01 * \coherentscalex, red]{};
\draw ($(enhanceTL)+(step2)+(0.130*\coherentscalex, 0.06*\coherentscalex)$) node[cross=0.01 * \coherentscalex, red]{};
\node[green] at ($(enhanceTL)+(step2)+(0.095*\coherentscalex, 0.095*\coherentscalex)$) {\fontsize{2.5}{4}\selectfont  $\checkmark$};



\coordinate (spycenter_fr3) at ($(enhanceTL)+(step2)+(0.095*\coherentscalex, 0.095*\coherentscalex)$);
\coordinate (spyposrel_fr3) at (-0.25*\coherentscalex, -0.3*\coherentscalex);
\coordinate (spypos_fr3) at ($(enhanceTR)+(spyposrel_fr3)$);
\spy [red, magnification=2.5] on (spycenter_fr3) in node at  (spypos_fr3);


\coordinate (step3) at (0.55*\coherentscalex,-0.8*\coherentscaley);

\draw[-stealth] ($(enhanceTL)+(step3)$) -- ++ (0, 0.2 * \coherentscalex) node[left] {\tiny Y};
\draw[-stealth] ($(enhanceTL)+(step3)$) -- ++ (0.2 * \coherentscalex, 0) node[below] {\tiny X};



\draw[line width = 2, ->] ($(enhanceTL)+(step2) + (0.05 * \coherentscalex, -0.05 * \coherentscalex)$) |- ($(enhanceTL)+(step3) + (-0.05 * \coherentscalex, 0.1 * \coherentscalex)$);


\filldraw[classcolor!20!white] ($(enhanceTL)+(step3)+(0.1*\coherentscalex, 0.11*\coherentscalex)$) circle (0.04 * \coherentscalex) ;
\filldraw[sub6color!30!white] ($(enhanceTL)+(step3)+(0.1*\coherentscalex, 0.1*\coherentscalex)$) circle (0.02 * \coherentscalex) ;
\filldraw[fr3color!30!white] ($(enhanceTL)+(step3)+(0.095*\coherentscalex, 0.095*\coherentscalex)$) circle (0.012 * \coherentscalex) ;


\filldraw[black] ($(enhanceTL)+(step3)+(0.0925*\coherentscalex, 0.0975*\coherentscalex)$) circle (0.0025 * \coherentscalex);

\filldraw[black] ($(enhanceTL)+(step3)+(0.1025*\coherentscalex, 0.1075*\coherentscalex)$) circle (0.0025 * \coherentscalex);
\filldraw[black] ($(enhanceTL)+(step3)+(0.0825*\coherentscalex, 0.1075*\coherentscalex)$) circle (0.0025 * \coherentscalex);
\filldraw[black] ($(enhanceTL)+(step3)+(0.1025*\coherentscalex, 0.0875*\coherentscalex)$) circle (0.0025 * \coherentscalex);
\filldraw[black] ($(enhanceTL)+(step3)+(0.0825*\coherentscalex, 0.0875*\coherentscalex)$) circle (0.0025 * \coherentscalex);

\coordinate (spycenter) at ($(enhanceTL)+(step3)+(0.0925*\coherentscalex, 0.0975*\coherentscalex)$);
\coordinate (spyposrel) at (-0.25*\coherentscalex, -0.7*\coherentscalex);
\coordinate (spypos) at ($(enhanceTR)+(spyposrel)$);
\spy [red] on (spycenter) in node at  (spypos);

 \begin{pgfonlayer}{fg}    % select the main layer
\draw[-stealth] (spypos)  -- ++(0.25*\boxwidth,0);% node[right, align=center] {Refined \\ location};

\end{pgfonlayer}


%phase links
\draw[-stealth, yellow!80!black] ($(FR1TR)!.7!(FR1BR)$) node[left] {$\phi$} --  ($(enhanceTL)!.25!(enhanceBL)$);
\draw[-stealth,yellow!80!black] ($(FR3TR)!.7!(FR3BR)$) node[left] {$\phi$} --  ($(enhanceTL)!.5!(enhanceBL)$);
\draw[-stealth,yellow!80!black, dashed] ($(FR2TR)!.7!(FR2BR)$) node[left] {$\phi$} --  ($(enhanceTL)!.75!(enhanceBL)$);



\end{tikzpicture}%
